Multiple Random Walks to Uncover Short Paths in Power Law Networks

Consider the following routing problem in the context of a large scale network $G$, with particular interest paid to power law networks, although our results do not assume a particular degree distribution. A small number of nodes want to exchange messages and are looking for short paths on $G$. These nodes do not have access to the topology of $G$ but are allowed to crawl the network within a limited budget. Only crawlers whose sample paths cross are allowed to exchange topological information. In this work we study the use of random walks (RWs) to crawl $G$. We show that the ability of RWs to find short paths bears no relation to the paths that they take. Instead, it relies on two properties of RWs on power law networks: 1) RW's ability observe a sizable fraction of the network edges; and 2) an almost certainty that two distinct RW sample paths cross after a small percentage of the nodes have been visited. We show promising simulation results on several real world networks.

==> Makefile <==
#

SRC=paper.tex references.bib algorithm.tex discussion.tex intro.tex paper.tex results.tex spanners.tex edges_in_St.tex

TARGET=paper.pdf
PDFLATEX=pdflatex
BIBTEX=bibtex

$(TARGET): $(SRC)
	$(PDFLATEX) $(@:.pdf=.tex)
	$(BIBTEX) $(@:.pdf=)
	$(PDFLATEX) $(@:.pdf=.tex)
	$(PDFLATEX) $(@:.pdf=.tex)

clean:
	\rm -f *.log *.aux *.blg *.bbl

veryclean:
	\rm -f *.log *.aux *.blg *.bbl $(TARGET)


==> spanners.tex <==
{\color{gray}
\subsection{Graph Spanners}

Given a graph $G=(V,E)$, a subgraph $G'=(V',E')$ is a $t$-spanner of $G$ if for
all $u,v \in V$, the following holds~\cite{PS89}:

\begin{equation}
	\label{eq:distuv}
	\frac{dist(u,v,G')}{dist(u,v,G)} \le t
\end{equation}

Sparse spanners that have low {\em stretch}, $t$, can be useful for routing in
scenarios described earlier.

We define $k$-$t$-spanner of $G=(V,E),S\subseteq V$ (where $S$ denotes the
{\small} set of vertices that want to find routes among each other) as follows:

A subgraph $G'=(V',E')$ is a $t$-$S$-spanner of $G$ w.r.t $S$ if for all $u,v
\in S$, the same inequality in \ref{eq:distuv} holds.

It is one thing to {\em find} a $t$-$S$-spanner $Z$ when the whole graph $G$ is
known, but it is another thing to construct $Z$ starting with limited
knowledge (of only neighbors). If the optimal or approximately-optimal spanner
is a subgraph of that constructed by the union of $k$ random walkers,
then it is ideal. The hard problems here are 
\begin{itemize}
\item To characterize the number of edges in the optimal $S$-$t$-spanner if $G$
were known.
\item To characterize the number of edges in the heuristic spanner constructed
by $k$ random walks.
\end{itemize}
}
